Uncertainty Quantification and Decomposition for LLM-based Recommendation

Despite the widespread adoption of large language models (LLMs) for recommendation, we demonstrate that LLMs often exhibit uncertainty in their recommendations. To ensure the trustworthy use of LLMs in generating recommendations, we emphasize the importance of assessing the reliability of recommendations generated by LLMs. We start by introducing a novel framework for estimating the predictive uncertainty to quantitatively measure the reliability of LLM-based recommendations. We further propose to decompose the predictive uncertainty into recommendation uncertainty and prompt uncertainty, enabling in-depth analyses of the primary source of uncertainty. Through extensive experiments, we (1) demonstrate predictive uncertainty effectively indicates the reliability of LLM-based recommendations, (2) investigate the origins of uncertainty with decomposed uncertainty measures, and (3) propose uncertainty-aware prompting for a lower predictive uncertainty and enhanced recommendation. Our source code and model weights are available at https://github.com/WonbinKweon/UNC_LLM_REC_WWW2025

==> 10.Trash.tex <==
%% intro
As LLMs have been adopted for real-world applications that can affect human behaviors, recent work has addressed the importance of assessing the reliability of answers generated by LLMs \cite{kuhn2022semantic, uncicl}.
In the literature, uncertainty quantification has gained traction as a perspective approach to quantitatively measure the reliability of responses generated by LLMs \cite{uncicl}.
Due to the intrinsic stochasticity and prompting scheme of LLMs, LLMs have uncertainty in their prediction; LLMs may generate false facts (i.e., hallucinations) \cite{llmunc4} and highly volatile answers for a single prompt \cite{kuhn2022semantic}.
In the recommendation task, similarly, we demonstrate LLMs generate volatile recommendations depending on the prompting scheme even with the same context information.
This is a key difference compared to the conventional CF models.
While the inspiring progress of estimating uncertainty mainly concentrated on the question-answering \cite{kuhn2022semantic} and the classification \cite{uncicl}, there is a lack of study on uncertainty of recommendation generated by LLMs.

Instruction-tuned foundation models \cite{gpt35,touvron2023llama,team2024gemma,jiang2023mistral} have shown remarkable performance for the zero-shot ranking task \cite{zeroshot1, zsc1}, enabling ranking the candidate items based on the context given in the textual prompt.
They further can be fine-tuned with the user history logged on the system \cite{tallrec,p5,collm}, utilizing the collaborative knowledge along with the content knowledge.

a systematic approach for (1) quantifying the predictive uncertainty of LLMs for recommendation, (2) investigating the relationship between the uncertainty and recommendation performance, and (3) enhancing recommendation performance through prompting schemes that result in lower uncertainty.

%% MA Table
\begin{table}[t]
\caption{Zero-shot ranking performance (NDCG@$K$) of large language models with various prompts on MovieLens 1M.}
\vspace{-0.2cm}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\toprule
 & \multicolumn{2}{c|}{Llama2-7B} & \multicolumn{2}{c|}{Gemma-7B} & \multicolumn{2}{c}{Mistral-7B} \\
Prompt & N@10 & N@20 & N@10 & N@20 & N@10 & N@20 \\
\midrule
\midrule
Fig.\ref{prompt1} (default) & 0.3038 & 0.4086 & 0.3310 & 0.4254 & 0.4179 & 0.4922 \\
Candidate [A] $\rightarrow$ Movie [A] & 0.2648 & 0.3751 & 0.3131 & 0.4143 & 0.4072 & 0.4845 \\
Candidate [A] $\rightarrow$ Candidate [1] & 0.2173 & 0.3451 & 0.2450 & 0.3706 & 0.2615 & 0.3850 \\
Candidate [A] $\rightarrow$ Candidate A & 0.2739 & 0.3823 & 0.2748 & 0.3862 & 0.3425 & 0.4542 \\
`\{item\}' $\rightarrow$ \{item\} & 0.2849 & 0.3901 & 0.2879 & 0.3965 & 0.4038 & 0.4849 \\
\midrule
Standard Deviation & 0.0323 & 0.0233 & 0.0337 &	0.0220 & 0.0676 & 0.0445 \\
\bottomrule
\end{tabular}}
\label{anal_prompt}
\vspace{-0.1cm}
\end{table}

%% origin figure
\begin{figure*}[ht!]
\centering
    \begin{minipage}[r]{0.215\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
          \includegraphics[width=1\textwidth]{figure/epoch_ml1m.png}
        \end{subfigure}
        % \vspace{-0.8cm}
        \caption*{(a)}
    \end{minipage}
    \begin{minipage}[r]{0.22\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
    \includegraphics[width=1\textwidth]{figure/size_ml1m.png}
    % \vspace{-0.1cm}
        \end{subfigure}
        \caption*{(b)}
        % \vspace{+0.1cm}
    \end{minipage}
    \begin{minipage}[r]{0.322\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
          \includegraphics[width=1\textwidth]{figure/hist_ml1m.png}
        \end{subfigure}
        % \vspace{+0.001cm}
        \caption*{(c)}
    \end{minipage}
    \begin{minipage}[r]{0.215\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
          \includegraphics[width=1\textwidth]{figure/cand_ml1m.png}
        \end{subfigure}
        % \vspace{+0.001cm}
        \caption*{(d)}
    \end{minipage}
    \caption{Analysis of fine-tuned ranking on MovieLens 1M. \%Pro. Unc. denotes the proportion of prompt uncertainty within the total uncertainty. For (d), the leave-one-out ground-truth item is \textit{not} guaranteed to be included in the candidate set.}
\vspace{-0.3cm}
\label{fig:analysis}
\Description{analysis}
\end{figure*}

%% prompt tables 2
\begin{table}[t]
\caption{Uncertainty-aware user history adjusting. TU, RU, and PU represent Total Uncertainty, Recommendation Uncertainty, and Prompt Uncertainty, respectively. \#Hist. denotes the average number of user history used for prompts. The ground-truth item is guaranteed to be included in the candidate set.}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccccc}
\toprule
model & prompt & N@10 & N@20 & TU & RU & PU & \#Hist. \\
\midrule
\midrule
\multicolumn{8}{c}{MovieLens 1M} \\
\midrule
\multirow{2}{*}{Llama2-7B} & default & 0.2881 & 0.3851 & 2.254 & 1.906 & 0.349 & 20 \\
 & unc.-aware & \textbf{0.3782} & \textbf{0.4345} & \textbf{1.714} & \textbf{1.386} & \textbf{0.328} & 20.46 \\
 \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.2987 & 0.3998 & 3.041 & 1.570 & 1.471 & 20 \\
 & unc.-aware & \textbf{0.3919} & \textbf{0.4717} & \textbf{2.034} & \textbf{0.837} & \textbf{1.196} & 20.86 \\
 \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.2815 & 0.4001 & 2.914 & 1.568 & \textbf{1.347} & 20 \\
 & unc.-aware & \textbf{0.3831} & \textbf{0.4843} & \textbf{1.956} & \textbf{0.573} & 1.383 & 19.41 \\
 \midrule
\multicolumn{8}{c}{Amazon Grocery} \\
 \midrule
\multirow{2}{*}{Llama2-7B} & default & 0.2784 & 0.3748 & 3.852 & 2.715 & \textbf{1.137} & 10 \\
 & unc.-aware & \textbf{0.3817} & \textbf{0.4582} & \textbf{2.378} & \textbf{1.173} & 1.205 & 9.97 \\
  \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.2302 & 0.4079 & 3.204 & 2.674 & 0.530 & 10 \\
 & unc.-aware & \textbf{0.3446} & \textbf{0.4341} & \textbf{1.798} & \textbf{1.314} & \textbf{0.484} & 9.81 \\
  \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.3135 & 0.3965 & 3.968 & 3.207 & \textbf{0.760} & 10 \\
 & unc.-aware & \textbf{0.3566} & \textbf{0.4498} & \textbf{2.502} & \textbf{1.304} & 1.198 & 10.02 \\
 \midrule
\multicolumn{8}{c}{Steam} \\
 \midrule
\multirow{2}{*}{Llama2-7B} & default & 0.7056 & 0.7202 & 1.804 & 1.250 & \textbf{0.554} & 20 \\
 & unc.-aware & \textbf{0.7199} & \textbf{0.7353} & \textbf{1.372} & \textbf{0.807} & 0.565 & 19.79 \\
  \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.7153 & 0.7274 & 1.553 & 1.119 & \textbf{0.434} & 20 \\
 & unc.-aware & \textbf{0.7294} & \textbf{0.7404} & \textbf{1.190} & \textbf{0.743} & 0.448 & 19.82 \\
  \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.7205 & 0.7508 & 1.496 & 1.041 & 0.455 & 20 \\
 & unc.-aware & \textbf{0.7315} & \textbf{0.7605} & \textbf{0.981} & \textbf{0.597} & \textbf{0.384} & 19.91 \\
 \bottomrule
\end{tabular}}
\label{tab:al_hist}
\vspace{-1em}
\end{table}

\begin{table}[t]
\caption{Uncertainty-aware candidate adjusting. TU, RU, and \%PU represent Total Uncertainty, Recommendation Uncertainty, and the proportion of Prompt Uncertainty, respectively. \#Cand. denotes the average number of candidate items used for prompts. The ground-truth item is \textit{not} guaranteed to be included in the candidate set.}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccccc}
\toprule
model & prompt & N@10 & N@20 & TU & RU & \%PU & \#Cand. \\
\midrule
\midrule
\multicolumn{8}{c}{MovieLens 1M} \\
\midrule
\multirow{2}{*}{Llama2-7B} & default & 0.0448 & 0.0638 & 2.492 & \textbf{0.822} & 67.01 & 20 \\
 & unc.-aware & \textbf{0.0564} & \textbf{0.0692} & \textbf{1.712} & 0.908 & \textbf{46.96} & 20.53 \\
  \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.0462 & 0.0574 & 2.175 & 0.854 & 60.76 & 20 \\
 & unc.-aware & \textbf{0.0566} & \textbf{0.0671} & \textbf{1.489} & \textbf{0.789} & \textbf{47.01} & 19.15 \\
  \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.0511 & 0.0612 & 1.989 & 0.790 & 60.27 & 20 \\
 & unc.-aware & \textbf{0.0578} & \textbf{0.0669} & \textbf{1.300} & \textbf{0.751} & \textbf{42.22} & 19.78 \\
 \midrule
\multicolumn{8}{c}{Amazon Grocery} \\
\midrule
\multirow{2}{*}{Llama2-7B} & default & 0.0477 & 0.0517 & 2.707 & \textbf{0.844} & 68.82 & 20 \\
 & unc.-aware & \textbf{0.0582} & \textbf{0.0632} & \textbf{2.317} & 0.959 & \textbf{58.61} & 20.01 \\
  \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.0455 & 0.0506 & 3.091 & 1.470 & 52.45 & 20 \\
 & unc.-aware & \textbf{0.0570} & \textbf{0.0602} & \textbf{2.726} & \textbf{1.344} & \textbf{50.70} & 20.07 \\
  \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.0506 & 0.0559 & 2.502 & 1.641 & 34.42 & 20 \\
 & unc.-aware & \textbf{0.0608} & \textbf{0.0670} & \textbf{1.900} & \textbf{1.592} & \textbf{16.19} & 19.61 \\
 \midrule
\multicolumn{8}{c}{Steam} \\
\midrule
\multirow{2}{*}{Llama2-7B} & default & 0.0516 & 0.0606 & \textbf{1.845} & \textbf{0.886} & 51.98 & 20 \\
 & unc.-aware & \textbf{0.0594} & \textbf{0.0714} & 1.848 & 1.031 & \textbf{44.21} & 19.61 \\
  \midrule
\multirow{2}{*}{Gemma-7B} & default & 0.0523 & 0.0621 & \textbf{1.639} & \textbf{0.751} & 54.20 & 20 \\
 & unc.-aware & \textbf{0.0619} & \textbf{0.0724} & 1.656 & 0.898 & \textbf{45.77} & 20.14 \\
  \midrule
\multirow{2}{*}{Mistrial-7B} & default & 0.0509 & 0.0641 & 1.526 & \textbf{0.638} & 58.21 & 20 \\
 & unc.-aware & \textbf{0.0610} & \textbf{0.0762} & \textbf{1.525} & 0.769 & \textbf{49.59} & 19.83 \\
 \bottomrule
\end{tabular}}
\label{tab:al_cand}
\vspace{-2em}
\end{table}

%%
This predictive uncertainty is the highest when LLMs predict uniform probability for all possible rankings.
In this case, LLMs generate highly volatile rankings since the predictive distribution $q(\pi_u|\mathcal{H}_u, \mathcal{C}_u)$ is smooth.
On the other hand, if LLMs predict a very large probability for one ranking $\pi_*$ and a marginal probability for the other $(|\mathcal{C}_u|!-1)$ rankings, the predictive uncertainty is low.
In this case, LLMs are likely to consistently generate the same ranking $\pi_*$ for multiple stochastic inferences.

==> 6.EXP_old.tex <==
% \begin{table}[t]
%  \renewcommand{\arraystretch}{0.6}
%  \caption{Data statistics after the preprocessing.}
%  \vspace{+0.1cm}
%   \begin{tabular}{ccccc}
%     \toprule
%     Dataset & \#Users & \#Items & \#Interactions & Sparsity \\
%     \midrule
%     MovieLens 1M & 6,040 & 3,883 & 1,000,207 & 95.74\% \\
%     Amazon Grocery & 21,027 & 18,857 & 358,602 & 99.91\% \\
%     Steam & 38,503 & 6,267 & 1,722,038 & 99.29\% \\
%     \bottomrule
%   \end{tabular}
%   \vspace{-0.3cm}
%   \label{tab:dataset}
% \end{table}

% In this section, we demonstrate the effectiveness of our uncertainty quantification framework.
% Effective uncertainty measures should indicate the reliability of the generated recommendations; recommendations with high uncertainty should be less likely to be correct.

\input{table/main_table}

\subsection{Experiment Setup}
\label{expsetup}
We provide a summary of the experiment setup due to limited space.
Please refer to the Appendix for the details about data statistics and fine-tuning. % including data statistics 
We provide an anonymous GitHub repository.\footnote{\url{anonymous}}

\subsubsection{\textbf{Evaluation metrics}}
Effective uncertainty measures should indicate the reliability of the generated recommendations; recommendations with higher uncertainty should be less likely to be accurate.
% Literature on uncertainty of classifiers \cite{kuhn2022semantic, verb1s} adopts AUROC to measure the probability that a randomly chosen correct prediction has a lower uncertainty than a randomly chosen incorrect prediction.
We adopt Kendall's $\tau$ ($\tau@K$) \cite{kendalltau} and Concordance Index (C@$K$) \cite{cindex} to assess whether a recommendation with lower uncertainty yields higher NDCG@$K$ than one with higher uncertainty.

\subsubsection{\textbf{Dataset}}
We use three real-world datasets, including MovieLens 1M\footnote{https://grouplens.org/datasets/movielens/}, Amazon Grocery \cite{amazon19}, and Steam \cite{sasrec}.
These publicly available datasets have representative text (e.g., title, description) for each item and have been widely used for LLM-based recommendation \cite{zeroshot1}.
% We adopt the 20-core setting for MovieLens 1M and Steam, and the 10-core setting for Amazon Grocery.
For each user's history, we hold out the last item for testing and the penultimate item for validation.
% The remaining items are used to construct $\mathcal{H}_u$.
% Data statistics after the preprocessing are presented in Table \ref{tab:dataset}.

\subsubsection{\textbf{Base large language models}}
We adopt three popular instruction-tuned foundation models including Llama2-7B \cite{touvron2023llama}, Gemma-7B \cite{team2024gemma}, and Mistral-7B \cite{jiang2023mistral} from Hugging Face \cite{wolf2019huggingface}.

\subsubsection{\textbf{Implementation details}}
\label{sec:implemetation}
We adopt two ranking scenarios: zero-shot and fine-tuned rankings.
For both scenarios. we set the maximum number of user history to 20 (MovieLens 1M, Steam) and 10 (Amazon Grocery).
The number of candidates is set to 20 for all datasets, and the leave-one-out ground-truth item is guaranteed to be included unless we note it separately.
We modify verbs and nouns for each dataset (e.g., $\texttt{"watch"} \rightarrow \texttt{"play"}$ and $\texttt{"movie"} \rightarrow \texttt{"game"}$ in Figure \ref{prompt1} for Steam).
We sample five prompts for each user, randomly assigning positions to candidate items for each of the five prompts.
The final ranking list $\pi_u^*$ is generated by sorting the average probability across the five prompts (i.e., $\mathbf{E}_{\mathcal{P}_u}[q(i|\mathcal{P}_u)]$ for $i \in \mathcal{C}_u$).
All experiments are conducted on a single NVIDIA A100-80GB.

\vspace{+0.1cm}
\noindent \textbf{Zero-shot Ranking.}
We use the pre-trained weights of LLMs distributed in Hugging Face.
The candidates are randomly retrieved, following the zero-shot LLM ranking setup \cite{zeroshot1}.
We additionally adopt GPT-3-Turbo (gpt-3.5-turbo-0125) \cite{gpt35}, a powerful baseline for zero-shot ranking \cite{liu2023chatgpt,zs2}.

\vspace{+0.1cm}
\noindent \textbf{Fine-tuned Ranking.}
For each dataset, we fine-tune LLMs with the low-rank adaptation (LoRA) \cite{hu2021lora} for 20 epochs (MovieLens 1M and Amazon Grocery) and 10 epochs (Steam).
The learning rate is set to 2e-5 and the weight decay is set to 1e-2.
For LoRA, we configure $r=16$, $\alpha=16$, and set the dropout rate to 5e-2.
The candidates are retrieved with BPR-MF \cite{bpr09}.
% user history $\mathcal{H}_u$ and the prompt in Figure \ref{prompt1}.
% the parameter efficient fine-tuning, we adopt 

\subsubsection{\textbf{Methods compared}}
We adopt various state-of-the-art and conventional methods to compute the total predictive uncertainty:
\begin{itemize}[leftmargin=*]
    \item \textbf{Label Probability \cite{cal17}}: It uses the probability associated with the predicted label (i.e., confidence).
    \item \textbf{Semantic Uncertainty \cite{kuhn2022semantic}}: It stochastically generates multiple answers with a single prompt, and counts the proportion of answers to estimate the predictive distribution, which is utilized for the predictive uncertainty.
    \item \textbf{Verb. 1S top-1 \cite{verb1s}}: It constructs prompts for models to explicitly produce their confidence (e.g., \texttt{"Provide the probability that your answer is correct (0.0 to 1.0)."}).
    \item \textbf{MC-Dropout \cite{mcdropout}}: It approximates BNNs with a single model and dropout. We obtain five generations with dropout for each prompt.
    \item \textbf{BNN \cite{bnndecompose}}: It uses an ensemble of multiple models and conducts Bayesian inference for generation. In the experiment, we utilize an ensemble of \textit{five} independently fine-tuned LLMs and thus it is not a direct competitor of this research line \cite{kuhn2022semantic}.
\end{itemize}
MC-Dropout and BNN are adopted only for the fine-tuned ranking task, as we cannot apply them on zero-shot LLMs.

\noindent \textbf{Inference overhead.}
The inference time of ours is nearly identical to Label Probability and Verb. 1S top-1, as the number of inferences for generation is the same.
Semantic Uncertainty, MC-Dropout, and BNN require five times more inferences compared to ours.

\subsection{Effectiveness of Uncertainty Measures}
\begin{figure}[ht!]
\centering
    \begin{minipage}[r]{0.46\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
          \includegraphics[width=1\textwidth]{figure/data_n20_ml1m.png}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}[r]{0.45\linewidth}
        \centering
        \begin{subfigure}{1\textwidth}
          \includegraphics[width=1\textwidth]{figure/data_tu_ml1m.png}
        \end{subfigure}
    \end{minipage}
\caption{Recommendation performance and total uncertainty of fine-tuned LLMs for each dataset.}
\label{fig:dataset}
\Description{dataset}
\vspace{-0.4cm}
\end{figure}
Table \ref{tab:main} shows the performance of total predictive uncertainty estimated by ours and the methods compared.
We observe that the predictive uncertainty indeed indicates the reliability of recommendation generated by LLMs, with C@20 of over 0.95 in Steam.
Ours and compared methods exhibit higher $\tau@K$ and C$@K$ for the fine-tuned ranking task than the zero-shot ranking task, as the LLMs are aligned with the ranking task via fine-tuning.
Notably, our uncertainty measures outperform baselines in 18 out of 21 cells, demonstrating the superiority in indicating the reliability of the generated recommendations.
Moreover, ours achieves comparable or even better performance compared to BNN, which utilizes an ensemble of five LLMs.
Figure \ref{fig:dataset} shows NDCG@20 and our total uncertainty of fine-tuned LLMs for each dataset.
LLMs exhibit lower total uncertainty on datasets with higher NDCG@20, supporting our claim that the total uncertainty indicates the reliability of the generated recommendation.
Therefore, the predictive uncertainty serves as an objective criterion for assessing the reliability of LLM-based recommendations, and can be further leveraged to develop various strategies aimed at enhancing user satisfaction.
